Improved power methods for computing eigenvalues of dual quaternion Hermitian matrices

This paper investigates the eigenvalue computation problem of the dual quaternion Hermitian matrix closely related to multi-agent group control. Recently, power method was proposed by Cui and Qi in Journal of Scientific Computing, 100 (2024) to solve such problem. Recognizing that the convergence rate of power method is slow due to its dependence on the eigenvalue distribution, we propose two improved versions of power method based on dual complex adjoint matrices and Aitken extrapolation, named DCAM-PM and ADCAM-PM. They achieve notable efficiency improvements and demonstrate significantly faster convergence. However, power method may be invalid for dual quaternion Hermitian matrices with eigenvalues having identical standard parts but distinct dual parts. To overcome this disadvantage, utilizing the eigen-decomposition properties of dual complex adjoint matrix, we propose a novel algorithm EDDCAM-EA which surpasses the power method in both accuracy and speed. Application to eigenvalue computations of dual quaternion Hermitian matrices in multi-agent formation control and numerical experiments highlight the remarkable accuracy and speed of our proposed algorithms.

==> references.tex <==

@inproceedings{c1,
  title={Stereo visual SLAM based on unscented dual quaternion filtering},
  author={Bultmann, Simon and Li, Kailai and Hanebeck, Uwe D},
  booktitle={2019 22th International Conference on Information Fusion (FUSION)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}

@article{qc1,
  title={Building a Robust Implementation of Bearing-only Inertial SLAM for a UAV},
  author={Bryson, Mitch and Sukkarieh, Salah},
  journal={Journal of Field Robotics},
  volume={24},
  number={1-2},
  pages={113--143},
  year={2007},
  publisher={Wiley Online Library}
}

@article{clif,
  title={Preliminary sketch of biquaternions},
  author={Clifford},
  journal={Proceedings of the London Mathematical Society},
  volume={1},
  number={1},
  pages={381--395},
  year={1871},
  publisher={Oxford University Press}
}

@article{Cadena2016,
  title={Past, present, and future of simultaneous localization and mapping: Toward the robust-perception age},
  author={Cadena, Cesar and Carlone, Luca and Carrillo, Henry and Latif, Yasir and Scaramuzza, Davide and Neira, Jos{\'e} and Reid, Ian and Leonard, John J},
  journal={IEEE Transactions on robotics},
  volume={32},
  number={6},
  pages={1309--1332},
  year={2016},
  publisher={IEEE}
}

@article{Cheng2016,
  title={Dual quaternion-based graphical SLAM},
  author={Cheng, Jiantong and Kim, Jonghyuk and Jiang, Zhenyu and Che, Wanfang},
  journal={Robotics and Autonomous Systems},
  volume={77},
  pages={15--24},
  year={2016},
  publisher={Elsevier}
}

@article{Cui2023,
  title={A power method for computing the dominant eigenvalue of a dual quaternion Hermitian matrix},
  author={Cui, Chunfeng and Qi, Liqun},
  journal={Journal of Scientific Computing},
  volume={100},
  number={1},
  pages={21},
  year={2024},
  publisher={Springer}
}

@article{Daniilidis1999,
  title={Hand-eye calibration using dual quaternions},
  author={Daniilidis, Konstantinos},
  journal={The International Journal of Robotics Research},
  volume={18},
  number={3},
  pages={286--298},
  year={1999},
  publisher={SAGE Publications}
}

@article{hec1,
  title={Standard dual quaternion optimization and its applications in hand-eye calibration and SLAM},
  author={Qi, Liqun},
  journal={Communications on Applied Mathematics and Computation},
  volume={5},
  number={4},
  pages={1469--1483},
  year={2023},
  publisher={Springer}
}

@article{hec2,
  title={A regularization-patching dual quaternion optimization method for solving the hand-eye calibration problem},
  author={Chen, Zhongming and Ling, Chen and Qi, Liqun and Yan, Hong},
  journal={Journal of Optimization Theory and Applications},
  volume={200},
  number={3},
  pages={1193--1215},
  year={2024},
  publisher={Springer}
}

@article{hec3,
  title={Dual quaternion operations for rigid body motion and their application to the hand-eye calibration},
  author={Wang, Xiao and Sun, Haoxiang and Liu, Chenglin and Song, Hanwen},
  journal={Mechanism and Machine Theory},
  volume={193},
  pages={105566},
  year={2024},
  publisher={Elsevier}
}

@inproceedings{hec4,
  title={Robust hand-eye calibration of an endoscopic surgery robot using dual quaternions},
  author={Schmidt, Jochen and Vogt, Florian and Niemann, Heinrich},
  booktitle={Pattern Recognition: 25th DAGM Symposium, Magdeburg, Germany, September 10-12, 2003. Proceedings 25},
  pages={548--556},
  year={2003},
  organization={Springer}
}

@article{hec5,
  title={Hand-eye calibration of SCARA robots using dual quaternions},
  author={Ulrich, M and Steger, C},
  journal={Pattern Recognition and Image Analysis},
  volume={26},
  pages={231--239},
  year={2016},
  publisher={Springer}
}

@article{hec6,
  title={Simultaneous robot-world and hand-eye calibration using dual-quaternions and Kronecker product},
  author={Li, Aiguo and Wang, Lin and Wu, Defeng},
  journal={Int. J. Phys. Sci},
  volume={5},
  number={10},
  pages={1530--1536},
  year={2010}
}

@article{Duan2023,
  title={On {R}ayleigh Quotient Iteration for Dual Quaternion Hermitian Eigenvalue Problem},
  author={Duan, Shan-Qi and Wang, Qing-Wen and Duan, Xue-Feng},
  journal={Mathematics},
  volume={12},
  number={24},
  year={2024}
}

@article{qc6,
  title={A comparative review of hand-eye calibration techniques for vision guided robots},
  author={Enebuse, Ikenna and Foo, Mathias and Ibrahim, Babul Salam Ksm Kader and Ahmed, Hafiz and Supmak, Fhon and Eyobu, Odongo Steven},
  journal={IEEE Access},
  volume={9},
  pages={113143--113155},
  year={2021},
  publisher={IEEE}
}

@article{Grisetti2010,
  title={A tutorial on graph-based SLAM},
  author={Grisetti, Giorgio and K{\"u}mmerle, Rainer and Stachniss, Cyrill and Burgard, Wolfram},
  journal={IEEE Intelligent Transportation Systems Magazine},
  volume={2},
  number={4},
  pages={31--43},
  year={2010},
  publisher={IEEE}
}

@article{RQI,
  title={Convergence analysis of inexact Rayleigh quotient iteration},
  author={Notay, Yvan},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={24},
  number={3},
  pages={627--644},
  year={2003},
  publisher={SIAM}
}

@article{mac,
  title={Distributed formation control of multi-agent systems using complex Laplacian},
  author={Lin, Zhiyun and Wang, Lili and Han, Zhimin and Fu, Minyue},
  journal={IEEE Transactions on Automatic Control},
  volume={59},
  number={7},
  pages={1765--1777},
  year={2014},
  publisher={IEEE}
}

@article{qc7,
  title={An overview of hand-eye calibration},
  author={Jiang, Jianfeng and Luo, Xiao and Luo, Qingsheng and Qiao, Lijun and Li, Minghao},
  journal={The International Journal of Advanced Manufacturing Technology},
  volume={119},
  number={1},
  pages={77--97},
  year={2022},
  publisher={Springer}
}

@article{d2,
  title={Singular values of dual quaternion matrices and their low-rank approximations},
  author={Ling, Chen and He, Hongjin and Qi, Liqun},
  journal={Numerical Functional Analysis and Optimization},
  volume={43},
  number={12},
  pages={1423--1458},
  year={2022},
  publisher={Taylor \& Francis}
}

@article{d3,
  title={Minimax principle for eigenvalues of dual quaternion Hermitian matrices and generalized inverses of dual quaternion matrices},
  author={Ling, Chen and Qi, Liqun and Yan, Hong},
  journal={Numerical Functional Analysis and Optimization},
  volume={44},
  number={13},
  pages={1371--1394},
  year={2023},
  publisher={Taylor \& Francis}
}

@article{Li2023,
  title={Eigenvalues and singular values of dual quaternion matrices},
  author={Qi, Liqun and Luo, Ziyan},
  journal={Pacific Journal of Optimization},
volume={19},
  number={2},
  pages={257--272},
  year={2023}
}

@article{Qi2022,
  title={Dual quaternions and dual quaternion vectors},
  author={Qi, Liqun and Ling, Chen and Yan, Hong},
  journal={Communications on Applied Mathematics and Computation},
  volume={4},
  number={4},
  pages={1494--1508},
  year={2022},
  publisher={Springer}
}


@article{Qi20231,
  title={Dual quaternion matrices in multi-agent formation control},
  author={Qi, Liqun and Wang, Xiangke and Luo, Ziyan},
  journal={arXiv preprint arXiv:2204.01229},
  year={2022}
}

@article{Qi2023,
  title={Dual quaternion matrices in multi-agent formation control},
  author={Qi, Liqun and Wang, Xiangke and Luo, Ziyan},
  journal={Communications in Mathematical Sciences},
  volume={21},
  number={7},
  pages={1865-1874},
  year={2023}
}



@article{qc8,
  title={Calibration of wrist-mounted robotic sensors by solving homogeneous transform equations of the form {AX= XB}},
  author={Shiu, Yiu Cheung and Ahmad, Shaheen},
journal={Department of Electrical and Computer Engineering Technical Reports. Paper 592.},
  year={1987},
url={https://docs.lib.purdue.edu/ecetr/592}
}
@article{qc9,
  title={A new technique for fully autonomous and efficient 3D robotics hand-eye calibration},
  author={Roger, YT and Lenz, RK},
  journal={IEEE Transactions onRobotics and Automation},
  volume={5},
  number={3},
  pages={345--357},
  year={1989}
}

@inproceedings{c4,
  title={Multiview registration via graph diffusion of dual quaternions},
  author={Torsello, Andrea and Rodola, Emanuele and Albarelli, Andrea},
  booktitle={CVPR 2011},
  pages={2441--2448},
  year={2011},
  organization={IEEE}
}

@article{wang2023dual,
  title={Dual r-rank decomposition and its applications},
  author={Wang, Hongxing and Cui, Chong and Liu, Xiaoji},
  journal={Computational and Applied Mathematics},
  volume={42},
  number={8},
  pages={349},
  year={2023},
  publisher={Springer}
}

@article{wei2024singular,
  title={Singular value decomposition of dual matrices and its application to traveling wave identification in the brain},
  author={Wei, Tong and Ding, Weiyang and Wei, Yimin},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={45},
  number={1},
  pages={634--660},
  year={2024},
  publisher={SIAM}
}

@article{Wei2013,
  title={Autonomous navigation of Mars probe using {X}-ray pulsars: modeling and results},
  author={Wei, Erhu and Jin, Shuanggen and Zhang, Qi and Liu, Jingnan and Li, Xuechuan and Yan, Wei},
  journal={Advances in Space Research},
  volume={51},
  number={5},
  pages={849--857},
  year={2013},
  publisher={Elsevier}
}

@article{c5,
  title={On the comparisons of unit dual quaternion and homogeneous transformation matrix},
  author={Wang, Xiangke and Zhu, Huayong},
  journal={Advances in Applied Clifford Algebras},
  volume={24},
  pages={213--229},
  year={2014},
  publisher={Springer}
}

@article{Zhang1997,
  title={Quaternions and matrices of quaternions},
  author={Zhang, Fuzhen},
  journal={Linear Algebra and its Applications},
  volume={251},
  pages={21--57},
  year={1997},
  publisher={Elsevier}
}

@article{qc10,
  title={Simultaneous robot/world and tool/flange calibration by solving homogeneous transformation equations of the form {AX= YB}},
  author={Zhuang, Hanqi and Roth, Zvi S and Sudhakar, Raghavan},
  journal={IEEE Transactions on Robotics and Automation},
  volume={10},
  number={4},
  pages={549--554},
  year={1994},
  publisher={IEEE}
}

@article{ling2022neumann,
  title={von Neumann type trace inequality for dual quaternion matrices},
  author={Ling, Chen and He, Hongjin and Qi, Liqun and Feng, Tingting},
  journal={arXiv preprint arXiv:2204.09214},
  year={2022}
}

@article{chen2024dual,
  title={Dual Complex Adjoint Matrix: Applications in Dual Quaternion Research},
  author={Chen, Yongjun and Zhang, Liping},
  journal={arXiv preprint arXiv:2407.12635},
  year={2024}
}





